On the Parallel Tower of Hanoi Puzzle: Acyclicity and a Conditional Triangle Inequality

A parallel variant of the Tower of Hanoi Puzzle is described herein. Within this parallel context, two theorems on minimal walks in the state space of configurations, along with their constructive proofs, are provided. These proofs are used to describe a {\sl denoising method}: a method for identifying and eliminating sub-optimal transfers within an arbitrary, valid sequence of disk configurations (as per the rules of the Puzzle). We discuss potential applications of this method to hierarchical reinforcement learning.

==> Algorithm/Denoising.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
	\begin{algorithm}[H]\label{algorithm::noiseReduction}
		% \SetLine
		\SetKwData{this}{this}
		\SetKwData{child}{child}
		\SetKwData{denoise}{denoise}

			\eIf{$\this.\child \neq \emptyset$}{
				$\this.{\tt child} = \List{N}{1}{m}$\;
			\While{ $\exists N_a,N_b \left(N_{a},N_{b} \in \this.{\tt child }
 				\textmd{ where Theorem} \ \ref{theorem::1} \ \textmd{or} \  \ref{theorem::2} \ applies\right)\ $}{ 
 					
 					\If{Theorem $1$ applies}{
		 				Apply the reduction method from Theorem \ref{theorem::1} to merge 
		 				the path trees rooted at $N_a,\ldots,N_b$ into a single path tree\;
 					}
 					\If{Theorem $2$ applies}{
		 				Apply the reduction method from Theorem \ref{theorem::2} to merge 
		 				the path trees rooted at $N_a,\ldots,N_{b-1}$ (or $N_{a+1},\ldots,N_{b}$) into a single path tree\; 					}
 				} %while
				\For{$N \in \this.\child$}{
					$N.\denoise()$\;
				}
				
			}{
				\Return{}\;
 			}
		\Return{}\;
		\caption{PathNode::\code{denoise}()}
	\end{algorithm}

	\begin{algorithm}[H]\label{algorithm::noiseReduction}
		% \SetLine
		\SetKwData{this}{this}
			$\this.\code{root}.\code{denoise}()$\;
			
		\Return{}\;
		\caption{PathTree::\code{denoise}()}
	\end{algorithm}



==> Algorithm/LevelSetJoin.tex <==
%!TEX root = ../../sToH.tex
\begin{algorithm}[]\label{algorithm::joinLevels}
		\SetKwData{base}{base}
		\SetKwData{BalanceRemainders}{Balance-Remainders}
		\SetKwData{center}{Center}
		\SetKwData{Extract}{Extract}
		\SetKwData{excludedPosts}{\ensuremath{\mathcal{E}}}
		\SetKwData{centerSet}{centerSet}
		\SetKwData{currentCenter}{current-center}
		\SetKwData{new}{new}
		\SetKwData{mapCenters}{Map-Centers}
		\SetKwData{mapCentersBase}{Map-Centers-Base}
		\SetKwData{newCenter}{newCenter}
		\SetKwData{stack}{Stack}
		\SetKwData{this}{this}
		\SetKwData{level}{level}
		\SetKwData{Height}{height}
		\SetKwData{invalidate}{invalidate}
		\SetKwData{Join}{join}
		\SetKwData{postScope}{postScope}
		\SetKwData{centerObject}{center}
		\SetKwData{result}{result}
		\SetKwData{restricted}{restricted}
		\SetKwData{Rebalance}{Rebalance}
	\KwIn{A pair of \code{LevelSet} objects $(X,Y)$}
	\KwOut{A \code{LevelSet} comprising levels centered around the current object}

	$Z \leftarrow \code{MatchBalancedLevels}(X,Y)$\;
	\tcp*[h]{The levels from $X$ and $Y$ that have been joined have been\\ removed in the \code{MatchBalancedLevels} method; join the \\ remaining levels}
	
	%$X \leftarrow X\backslash(X\cap Z)$\;
	%$Y \leftarrow Y\backslash(Y\cap Z)$\;
	
	%\tcp*[h]{Join the remaining levels}
	
	$W \leftarrow \code{MatchUnbalancedLevels}(X,Y)$\;
		
	
	
	\Return{$Z+W$}\;
	\caption{\code{LevelSet::Join$(\code{LevelSet}\ X, \code{LevelSet}\ Y)$}}
\end{algorithm}


==> Algorithm/joinBalancedLevels.tex <==
%!TEX root = ../sToH.tex
\begin{algorithm}[]\label{algorithm::joinBalancedLevels}
		\SetKwData{base}{base}
		\SetKwData{BalanceRemainders}{Balance-Remainders}
		\SetKwData{center}{Center}
		\SetKwData{Extract}{Extract}
		\SetKwData{excludedPosts}{\ensuremath{\mathcal{E}}}
		\SetKwData{centerSet}{centerSet}
		\SetKwData{currentCenter}{current-center}
		\SetKwData{new}{new}
		\SetKwData{mapCenters}{Map-Centers}
		\SetKwData{mapCentersBase}{Map-Centers-Base}
		\SetKwData{newCenter}{newCenter}
		\SetKwData{stack}{Stack}
		\SetKwData{this}{this}
		%\SetKwData{level}{level}
		\SetKwData{Height}{height}
		\SetKwData{invalidate}{invalidate}
		\SetKwData{Join}{join}
		\SetKwData{postScope}{postScope}
		\SetKwData{centerObject}{center}
		\SetKwData{result}{result}
		\SetKwData{restricted}{restricted}
		\SetKwData{Rebalance}{Rebalance}
	\KwIn{A \code{LevelSet} pair $(X,Y)$}
	\KwOut{A \code{LevelSet} $Z$}
	
	$X\leftarrow \List{x}{0}{u}$\;
	$Y\leftarrow \List{y}{0}{v}$\;
	$m \leftarrow \min(u,v)$\;
	
	\For{$i:\ 1 \to m$}{
		$\eta_i \leftarrow \min(x_i,y_i)$\;	
		\For{$j:\ 1 \to \eta_i$}{
			$x$ $\leftarrow$ a level from $X$ of height $i$\;
			$y$ $\leftarrow$ a level from $Y$ of height $i$\;
			$z$ $\leftarrow$ $\join{x}{y}$\;
			$Z_{i}.\code{insert}(z)$\;
			$X.\code{remove}(x)$\;
			$Y.\code{remove}(y)$\;
		}	
	}
	\Return{$Z = \parentheses{0,\listKernel{Z}{1}{m}}$}\;
	\caption{\code{LevelSet::JoinBalancedLevels$(\code{LevelSet}\ X, \code{LevelSet}\ Y)$}}
\end{algorithm}


==> Algorithm/joinLevels.tex <==
%!TEX root = ../../sToH.tex
\begin{algorithm}[]\label{algorithm::joinLevels}
		\SetKwData{base}{base}
		\SetKwData{BalanceRemainders}{Balance-Remainders}
		\SetKwData{center}{Center}
		\SetKwData{Extract}{Extract}
		\SetKwData{excludedPosts}{\ensuremath{\mathcal{E}}}
		\SetKwData{centerSet}{centerSet}
		\SetKwData{currentCenter}{current-center}
		\SetKwData{new}{new}
		\SetKwData{mapCenters}{Map-Centers}
		\SetKwData{mapCentersBase}{Map-Centers-Base}
		\SetKwData{newCenter}{newCenter}
		\SetKwData{stack}{Stack}
		\SetKwData{this}{this}
		\SetKwData{level}{level}
		\SetKwData{Height}{height}
		\SetKwData{invalidate}{invalidate}
		\SetKwData{Join}{join}
		\SetKwData{postScope}{postScope}
		\SetKwData{centerObject}{center}
		\SetKwData{result}{result}
		\SetKwData{restricted}{restricted}
		\SetKwData{Rebalance}{Rebalance}
	\KwIn{A \code{LevelSet} pair $(X,Y)$}
	\KwOut{A \code{LevelSet} $Z$}

	$Z' \leftarrow \code{joinBalancedLevels}(X,Y)$\;
	\tcp*[h]{The levels from $X$ and $Y$ that have been joined have been removed in the \code{joinBalancedLevels} method; join the  remaining orthogonal LevelSets}
	
	%$X \leftarrow X\backslash(X\cap Z)$\;
	%$Y \leftarrow Y\backslash(Y\cap Z)$\;
	
	%\tcp*[h]{Join the remaining levels}
	
	$Z'' \leftarrow \code{joinUnbalancedLevels}(X,Y)$\;
		
	
	
	\Return{$Z = Z'+Z''$}\;
	\caption{\code{LevelSet::joinLevels$(\code{LevelSet}\ X, \code{LevelSet}\ Y)$}}
\end{algorithm}


==> Algorithm/joinUnbalancedLevels.tex <==
%!TEX root = ../sToH.tex
\begin{algorithm}[]\label{algorithm::joinUnbalancedLevels}
		\SetKwData{base}{base}
		\SetKwData{BalanceRemainders}{Balance-Remainders}
		\SetKwData{center}{Center}
		\SetKwData{Extract}{Extract}
		\SetKwData{excludedPosts}{\ensuremath{\mathcal{E}}}
		\SetKwData{centerSet}{centerSet}
		\SetKwData{currentCenter}{current-center}
		\SetKwData{new}{new}
		\SetKwData{mapCenters}{Map-Centers}
		\SetKwData{mapCentersBase}{Map-Centers-Base}
		\SetKwData{newCenter}{newCenter}
		\SetKwData{stack}{Stack}
		\SetKwData{this}{this}
		\SetKwData{level}{level}
		\SetKwData{Height}{height}
		\SetKwData{invalidate}{invalidate}
		\SetKwData{Join}{join}
		\SetKwData{postScope}{postScope}
		\SetKwData{centerObject}{center}
		\SetKwData{result}{result}
		\SetKwData{restricted}{restricted}
		\SetKwData{Rebalance}{Rebalance}
	\KwIn{An orthogonal \code{LevelSet} pair $(X,Y)$}
	\KwOut{A \code{LevelSet} $Z$}

	$X\leftarrow \List{x}{0}{u}$\;
	$Y\leftarrow \List{y}{0}{v}$\;
	$m \leftarrow \min(|X|,|Y|)$\;
	
	\tcp*[h]{Join levels from $X$ and $Y$ of unequal heights until a level set of minimum order is empty}
	
	\For{$i:1\to m$}{
		$\lambda$ $\leftarrow$ level of maximum height in $X\cup Y$\;
		\If{$\lambda \in X$}{ 
			$\mu \leftarrow$  a level of minimum height in $Y$\;
			$z \leftarrow \join{\lambda}{\mu}$\;
			$X.\code{remove}(\lambda)$\;
			$Y.\code{remove}(\mu)$\;
		}
		\ElseIf{$\lambda \in Y$}{
			$\mu \leftarrow$  a level of minimum height in $X$\;
			$z \leftarrow \join{\mu}{\lambda}$\;
			$X.\code{remove}(\mu)$\;
			$Y.\code{remove}(\lambda)$\;
		}
		$Z_{\lambda}.\code{insert}(z)$\;
	}
	\Return{$Z = \parentheses{0,\listKernel{Z}{1}{\max(u,v)}}$}\;
	\caption{\code{LevelSet::joinUnbalancedLevels$(\code{LevelSet}\ X, \code{LevelSet}\ Y)$}}
\end{algorithm}


==> ConstructingREG/REGNaught.tex <==
%!TEX root = ../sToH.tex

==> Definition/ClusterWalkConcatenation.tex <==
% !TEX root = ../MLNotes.tex
\begin{definition}[Concatenating Cluster Walks]\label{definition::clusterWalkConcatenation}
	Let $\path$ and $\pathTwo$ be cluster walks where 
	\[
	\path=\List{1}{m}{A}
	\] and
	\[
	
	\]
\end{definition}


==> Proof/1.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
\begin{proof}\label{proof::1}
	Assume the notation within the hypotheses of the Theorem. 
	We will show that for any walk $\clusterSequence{\nu}{A}{B}$ where $\nu \nsubseteq \clusterSetOfCluster{j}{C}$,
there exists a walk
\clusterSequence{\mu}{A}{B} with the property that $\mu \subseteq \clusterSetOfCluster{j}{C}$ and
$\numberOfStates{\nu}>\numberOfStates{\mu}$.

	Assume the $i$-grading of $\nu$ is 
	$$\sequenceDecomposition{\nu}{j} = \List{C}{1}{m}$$  where the cluster $C= C_1 = C_m$, and $m > 2$. Let 
	\[
	 \nu = \sum_{C_a\in\sequenceDecomposition{i}{\nu}}\nu_a
	\] be the $i$-decomposition of $\nu$ where
	\[
	 \nu_a = \List{\alpha}{a,1}{a,l(a)}
	\] for $a\in\nSet{m}$.
	For $a > 1$, the equality
	%image  of the first sublist element of $\nu_a$ under the translative map $\translativeMapNotation\colon C_a \to C$ equals the last sublist element of $\nu_{a-1}$:  
	$$\Translate{\alpha_{a,1}}{C_a}{C} = \alpha_{a-1,l(a-1)}$$ holds. 
If we define 
\[
\nu'_a = \List{\alpha}{a,2}{a,l(a)}, 
\] for each $a>1$, then we can construct the cluster walk 
	\[
	 \mu = \mu_1 + \sum_{1< a \leq m} \mu_a
	\] where $\mu_1 = \nu_1$, and 
	\[
	   \mu_a = \Translate{ \nu'_a}{C_h}{C}
	\] for $1<a \leq m$. The walk $\mu$ is contained in $\clusterSetOfCluster{j}{C}$ and $\numberOfStates{\mu} =
\numberOfStates{\nu}-(m-1)$.
	
\end{proof}


==> Proof/2.tex <==
% !TEX root = ../pToH.tex
\begin{proof}\label{proof::2}

	Assume the notation and hypotheses within the theorem statement.
	
	The clusters $A$ and $B$ form a $\clusterPair[j]{A}{B}$ index $j$ under the assumptions.  
	%By way of contradiction, assume that $\nu$ is a minimal cluster walk of index $n$ that connects $\alpha$ and $\beta$, and that $\nu$ is not contained within $\clusterSetOfCluster{n}{A}\cup \clusterSetOfCluster{n}{B}$. Furthermore, assume that the $j$-grading of $\nu$ is $$\sequenceDecomposition{j}{\nu} =\left(A, \listKernel{C}{1}{m}, B\right)$$ where  $m\geq 1$.
	
	By Theorem \ref{theorem::1}, we can also assume that 
	\begin{enumerate}[i.]
		\item the  cluster walk $\nu$ is contained in the cluster \canonicalCluster{a}{1}{j-1} of index $j-1$, and
		\item the cluster walk \sequenceDecomposition{j}{\nu} is acyclic.
	\end{enumerate}
	 We will construct a walk $\mu$ that is contained
in $\clusterSetOfCluster{n}{A}\cup \clusterSetOfCluster{n}{B}$ where $\numberOfStates{\mu}~=~\numberOfStates{\nu}-m$.

	

	We will argue inductively on $m$.  Assume $m=1$, and let $C=C_1=\canonicalCluster{a}{1}{j-1}{\bf c}$ where  
$c\neq a$ and $c\neq b$. Let $\nu_A + \nu_C + \nu_B$ be the $j$-decomposition of $\nu$.  Furthermore,  assume that the subwalk 
$$\nu_A =
\List{\alpha}{1}{x},$$ 
 the subwalk 
 $$\nu_C =
\List{\gamma}{1}{z},$$  and the subwalk  
$$\nu_B = \List{\beta}{1}{y}.$$

The following conditions hold within the images of $\nu_A$ and $\nu_C$ under the reflective map $\reflectiveMap[j]{b}{c}$:
\begin{enumerate}[i.]
	\item the cluster $\reflect[j]{\alpha_1}{b}{c} = \alpha_1$ by assumption; 
	%as $\alpha_1 = \canonicalCluster{a}{1}{j-1}{\bfa}^{n-j+1}$ and $a\notin\{b,c\}$;
	\item if we assume that $$\gamma_z = \canonicalCluster{a}{1}{j-1}\textbf{c}\canonicalCluster{a}{j+1}{n},$$ then the image $$\reflect[j]{\gamma_z}{b}{c} =  \canonicalCluster{a}{1}{j-1}\textbf{b}\canonicalCluster{a}{j+1}{n} = \beta_1;$$
	\item the image $ \reflect[j]{\nu_C}{b}{c}$ is contained in $\clusterSetOfCluster{n}{B}$.
\end{enumerate}

  Thus, we can construct a cluster walk using the images of the subwalks $\nu_A$ and $\nu_B$ under this reflective mapping as follows: let us define
	\[
	 \mu = \reflect[j]{\nu_A+\nu_C}{b}{c} + \mu_B
	\] where $\mu_B = \List{\beta}{2}{y}$.
	This walk is contained in $\clusterSetOfCluster{n}{A}\cup \clusterSetOfCluster{n}{B}$, and  $\numberOfStates{\mu} = \numberOfStates{\nu}-1$.

	We can now proceed inductively on the number of intermediate clusters.  For $m> 1$, we  apply the above construction to the subwalk contained in $A \cup C_1 \cup C_2$;  this construction yields a valid walk
$\mu'$ where $\sequenceDecomposition{j}{\mu'} = \left(A,C_2, \ldots, C_m,B\right)$, and   $ \numberOfStates{\mu'}=
\numberOfStates{\nu}-1$; the inductive assumption is that $\mu'$ can be further reduced (if necessary) to eliminate the $(m-1)$ intermediate clusters $\List{C}{2}{m}$, and the resulting construction will be contained in $\clusterSetOfCluster{n}{A}\cup \clusterSetOfCluster{n}{B}$ as desired.

\end{proof}


==> Proof/3.tex <==
% !TEX root = ../main.tex
\begin{proof}\label{proof::3}
		Assume the notation and hypotheses within the statement of the theorem.
		We can assume that $\sequenceDecomposition{1}{\Path} = ({\bf 0},{\bf 1})$ according to  Theorem
\ref{theorem::2}. For any $p \geq 3$, we'll define $\tau = \translativeMapExtended{\Path}{K_p},$ which can be
written as
\[
	\tau  = \tau({\bf 0}^n,{\bf 0}^{n-k_p}{\bf x}^{k_p}) + \tau({\bf 0}^{n-k_p}{\bf
x}^{k_p},{\bf 1}^{n}),
\] If $x=0$, then the condition $2$ ensures that at least $M(k_p,p)$ transfers are included in both $\tau({\bf 0}^n,{\bf
0}^{n-k_p}{\bf x}^{k_p})$ and $\tau({\bf 0}^{n-k_p}{\bf
x}^{k_p},{\bf 1}^{n})$. Moreover, each
transfer of the disk of index within $\cup_{q<p} K_q$ generates a repeated element within $\tau$; as
$\numberOfTransfers{\Path} = \numberOfTransfers{\tau}$, the result follows induction on $p$.
%  	\end{enumerate}
\end{proof}


==> Proof/BalanceBandCorrectness.tex <==
\begin{proof}\label{proof::balanceBandHalting}
 
 (Sketch)  After iteration $i$, $c^{(i)}_i = 0$. Thus, no new values of $i+1$ can be created during any later iteration.  
 
\end{proof}


==> Proof/BalanceBandHalting.tex <==
\begin{proof}\label{proof::balanceBandHalting}
 
 (Sketch)  After iteration $i$, $c^{(i)}_i = 0$. Thus, no new values of $i+1$ can be created during any following iteration.  
 
\end{proof}


==> Proof/ClusterMappingsOfSequences.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
\begin{proof}\label{proof::clusterMappingsOfSequences}	\begin{enumerate}[i.] 
		\item   Let $\Path$ satisfy the hypotheses of (i.) in the lemma statement where  $\Path = \left(A_l\right)_{l=1}^{m}$
 Fix $B\in \clusterSet{i}$ where $i \in \nSet{j}$.  If $A_l = A_{l+1}$ where $A_l\in \clusterSetOfCluster{j}{C_a}$, then
it follows $\Translate{ A_l}{C_a}{B} = \Translate{A_{l+1} }{C_a}{B}$.  If $\clusterPair[k]{A_l}{A_{l+1}}$ for some fixed $k$, then 
			\begin{enumerate}
	        		\item[a.]if $k\leq i$, then $\Translate{ A_l}{C_a}{B} = \Translate{A_{l+1}
}{C_a}{B}$; 
	        		\item[b.]otherwise, if $k> i$ then $\clusterPair[k]{\Translate{
A_l}{C_a}{B}}{\Translate{A_{l+1} }{C_a}{B}}$.
			\end{enumerate}	
			
			
			
				
		\item Let $\rho$ satisfy the hypotheses of (ii.) in the lemma statement where $$\rho = \List{A}{1}{m},$$ and the cluster $A = \canonicalCluster{a}{1}{i-1}$.   For each $l\in \nSet{m}$, if $A_l = A_{l+1}$, then
$\reflect[i]{ A_l}{q}{r} = \reflect[i]{A_{l+1} }{q}{r}$.  If $A_l$ and $A_{l+1}$ form a cluster pair $\clusterPair[k]{A_l}{A_{l+1}}$ for some $k$, then the index $k\geq i$ as per the lemma conditions.   Assume that
$$A_l = \canonicalCluster{a}{1}{i-1}\canonicalCluster{a}{i}{k-1}{\bf d}\canonicalCluster{a}{k+1}{n},$$ 
and 
$$A_{l+1} = \canonicalCluster{a}{1}{i-1}\canonicalCluster{a}{i}{k-1}{\bf e}\canonicalCluster{a}{k+1}{n},$$  
where $d\neq e$. Under the assumption of adjacency, the post value $a_h \notin\{d,e\}$ for all $h>k$.  
We will denote the images 
$$\reflect[i]{A_l}{q}{r} = \canonicalCluster{a}{1}{i-1}\canonicalCluster{a'}{i}{k-1}{\bf d'}\canonicalCluster{a'}{k+1}{n}$$ 
and 
$$\reflect[i]{A_{l+1}}{q}{r} = \canonicalCluster{a}{1}{i-1}\canonicalCluster{a'}{i}{k-1}{\bf e'}\canonicalCluster{a'}{k+1}{n}.$$ 
We will now argue by cases.
	\begin{enumerate}[a.]
	  \item$\{d,e\} =  \{q,r\}$:  Without loss of generality, assume  $d = q$, and   $e = r$. Then, the post value  $d'=e$, and the post value $e'=d$.  Furthermore, as the post value $a_h\notin \{q,r\}$ for $h>k$, the post value $a'_{h} = a_h$; thus, the post value $a'_h\notin\{q,r\}$.  
 
 	 \item$|\{d,e\} \cap \{q,r\}| = 1$: Without loss of generality, assume $d=q$ and $e\notin\{q,r\}$; thus, we have $d' = r$.  As
 	 %\footnote{Note that if $k<i$, then the necessary condition $d'=r$ is not satisfied. Thus, the condition $\sequenceDecomposition{i-1}{\rho} = A$ is necessary.} 
 	  $e \notin \{q,r\}$,  we have  $e' = e \notin\{q,r\}$.
	  As none of the post values $a_h \in \{q,e\}$ for $h>k$, none of the post values $a'_h\in \{r,e\}$ (if $a'_h = r$, then $a_h = q$). 
	  %An analogous argument applies when $d \notin \{q,r\}$ and  $e \in \{q,r\}$.
 	
	 \item$|\{d,e\} \cap \{q,r\}| = 0$:  If $\{d,e\} \cap \{q,r\} = \emptyset$, then $d' = d$ and $e'=e$.  For each $h>k$, we have $a_h\notin\{d,e\}$. If $a_h\in \{q,r\}$, then $a'_h \in \{q,r\}$; otherwise, we have $a'_h = a_h$.  In both cases, we have $a'_h \notin \{d,e\}$. 	 
	\end{enumerate}
	
	In all three cases, we conclude that the images $\reflect[i]{A_l}{q}{r}$ and $\reflect[i]{A_{l+1}}{q}{r}$ form a $k$-pair.
	
\end{enumerate}
\end{proof}

==> Proof/IntermediateTowerBound.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
\begin{proof}\label{proof::intermediateTowerBound}
		Assume the notation and hypotheses within the statement of the theorem, and let $\clusterWalk{\Path}{A}{B} = \sum_{0\leq w < m}\alpha_w$.   
		
		The proof is by induction on $y$.
		
		When $y=1$, we have a cluster path connecting a tower of $n$ disks from post $a$ to post $b$; if $c(1) = 1$ (equivalently, if $A = B$), then $$\numberOfTransfers{\Path} \geq (1-1)\fsBound{n}{1} = 0.$$  If $c(1)>1$, then, for each $v\in \nSet{c(1)}$, the subpath connecting $\alpha_{v}$ and $\alpha_{v+1}$ contributes $\fsBound{n}{r_q}$ transfers to the path length; thus
		\[
		\numberOfTransfers{\Path} \geq \sum_{v\in \nOpenSet{c(1)}}\fsBound{n}{r_1} = (c(q)-1)\fsBound{n}{r_1}
		\] as required.
	
		Assume the bound holds for $y\geq 1$; and let $\mathcal{K} = \left(K_q\right)_{q=1}^{y+1}$ be a set partition of $\setOfDisks$ of order $y+1$.  Define $\tau = \extendedTranslativeMapNotation(\Path ;K_{y+1})$.  Each of the disks in $\mathcal{K}\backslash K_{y+1}$ contribute at least
		$
		 \sum_{1\leq q \leq y }\parentheses{c(q)-1}\fsBound{k_q}{r_q}
		$ transfers to the sequence length (which translate to repeated configurations in $\tau$).  By the inductive assumption, there are at least
		$
		 \sum_{1\leq q \leq y }\parentheses{c(q)-1}\fsBound{k_q}{r_q}
		$ such transfers.
		
		 We can decompose the cluster walk $\tau$ as
		\[
		\tau =\sum_{1\leq v < c(y+1)}\clusterWalk{\tau}{\alpha_{v}}{\alpha_{v+1}};
		\]  under the assumptions in (\ref{intermediateTowerCondition}), there are $\parentheses{c(y+1)-1}\fsBound{k_{y+1}}{r_{y+1}}$ transfers generated by the disks in $K_{y+1}$.
		

\end{proof}


==> Proof/JoinPropertiesProof.tex <==
% !TEX root = ../main.tex
\begin{proof}
	\begin{enumerate}[i.]
		\item All levels in $\mathcal{R}_{X-H,Y-H}$ are of the form $\join{x}{y}$ (precluding the existence of levels of height $0$).  Moreover, as $\height{\join{x}{y}} \geq \height{x}$ and $\height{\join{x}{y}} \geq \height{y}$, it follows that both $X-H \prec \mathcal{R}_{X-H,Y-H}$ and $Y-H \prec \mathcal{R}_{X-H,Y-H}$.
		\item Assume $X = \List{0}{u}{x}$, $Y = \List{0}{u}{y}$, and $Z =  \List{0}{u}{z}$.  Moreover, assume $Z\prec X$ and $Z\prec Y$.  
		Assume that $\join{X}{Y} = 2Q = \left(0,\listKernel{0}{u}{q}\right) = 2H +  \mathcal{R}_{X-H,Y-H}$ where
		\[
			H = \List{0}{u}{\eta}
		\] and 
		\[
		\mathcal{R}_{X-H,Y-H} = \List{0}{u}{\rho};
		\] thus, $q_i = \eta_i + \rho_{i+1}$. Let $X-H = \List{0}{u}{\chi}$,  and let $Y-H = \List{0}{u}{\omega}$.
		By construction, we have that $\chi_c>0 \implies~\omega_c~=0~$, and $\omega_c>0 \implies \chi_c = 0$.  		

		
		
		By way of contradiction, assume that $2Z \nprec \join{X}{Y}$. Let $\phi$ be the smallest index where
		\[
		\sum_{0\leq i \leq \phi}q_i > \sum_{0\leq i \leq \phi} z_i,
		\]  and, without loss of generality, assume that $\omega_{\phi+1}>0$.
		
		We have 
		\begin{alignat}{2}
			\sum_{0 \leq i \leq \phi} z_i 	&< \sum_{0 \leq i \leq \phi} q_i 	\notag \\
								&= \sum_{0 \leq i \leq \phi} \left( \eta_i + \rho_{i+1}\right) \notag \\
								&=  \sum_{0 \leq i \leq \phi} \eta_i  + \rho_0 + \sum_{1 \leq i \leq \phi+1} \rho_i \notag \\
								& \leq \sum_{0 \leq i \leq \phi} \eta_i + \sum_{0 \leq i \leq \phi+1} \chi_i \notag \\ 
								& = \sum_{0 \leq i \leq \phi} x_i+ \chi_{\phi+1} \notag  \\ 
								&= \sum_{0 \leq i \leq \phi} x_i; \notag
		\end{alignat} thus, $Z\nprec X$.
		
	\end{enumerate}	
\end{proof}

==> Proof/LevelOneBound.tex <==
% !TEX root = ../main.tex
\begin{proof}\label{proof::levelOneBound}
	There are $|\mathfrak{L}|$ choices for the first value and $|\mathfrak{R}|$ choices for the second value in any ordered pair in 
	$\mathfrak{L} \times \mathfrak{R}$.   However, if $q\in\mathfrak{L}\cap\mathfrak{R}$, then a level of height $1$ to and from post $q$ cannot exist (a disk with the same source and target post is either static or transfers at least twice).  Moreover, for any $r \in \mathfrak{L} \cap \mathfrak{R}$ with $ r\neq q$, at most one level of height $1$ that connects post $q$ and $r$ can exist (by the parenthesis structure of the Puzzle).  Thus, there are at most 
	\[
	|\mathfrak{L}| |\mathfrak{R}| - \left[ {|\mathfrak{L} \cap \mathfrak{R}| \choose 1} + {|\mathfrak{L} \cap \mathfrak{R}| \choose 2} \right]
	\] as desired.
\end{proof}

==> Proof/PrecursorToTheorem3.tex <==
\begin{proof}\label{proof::precursorToTheorem3}
 	Let $\sequenceDecomposition{j}{\sigma}$
\end{proof}


==> Proof/RTreePlus.tex <==
% !TEX root = ../main.tex
\begin{proof}
	Let $X = \List{0}{u}{x}$,$Y = \List{0}{u}{y}$,  $W = \List{0}{u}{w}$, and $Z = \List{0}{u}{z}$. For each $h\geq 0$, we have
	\[
	\sum_{0 \leq i \leq h} z_i \geq 
	\sum_{0 \leq i \leq h} \left(x_i+y_i\right) = 
	\sum_{0 \leq i \leq h} x_i  + \sum_{0 \leq i \leq h} y_i \geq  
	\sum_{0 \leq i \leq h} w_i  + \sum_{0 \leq i \leq h} y_i = 
	 \sum_{0 \leq i \leq h}  \geq \left(w_i+y_i\right)
	\] as $Z \prec X+Y$ and $X\prec W$.
\end{proof}

==> Proof/ReflectiveCorrectness.tex <==
\begin{proof}\label{proof::reflectiveCorrectness}
	 We consider each case in the above order.
		\begin{enumerate}
		 \item[i.] Firstly, we can apply the mapping $\reflectiveMap{1}{a}{b}$ to $(\alpha_w)_{w=r+1}^{s}$ as no active boundary
intervals in $\omega$ (other than perhaps $B$ and $X$) 
		 have a post value in $\{a,b\}$.  If $\postValueOfInterval{X}\in\{a,b\}$, then the fact that all other boundary intervals
		 $Z$ have post values in $\posts \backslash \{a,b\}$ implies  that
$\transferWithIntervals{\reflectiveMapping(X)}{\postValueOfInterval{\reflectiveMapping(X)}}{\postValueOfInterval{Y}}{Y}{j}$ is a valid
transfer according 
		 to the rules of the puzzle.  Moreover, as no active intervals with post values in $\{a,b\}$ are covered
		 by static intervals with post values in the same set, the restriction of application of the 
		 mapping to active intervals does not introduce intervals covered by intervals with the same post value
		 within  $(\reflectiveMapping(\alpha_w))_{w=r+1}^{s}$ 
		 
		 After this application of the mapping at $\alpha_{r+1}$ we have
		 $\postValueOfInterval{A} = \postValueOfInterval{B}$ and thus we can remove $\lambda_r$ from the resulting transfer
sequence.
		 
		 \item[ii.] Similar to the first case, we can apply the mapping $\reflectiveMap{1}{x}{y}$ to $(\alpha_w)_{w=r+1}^{s}$ as no
active boundary intervals in $\omega$ (other than perhaps $B$ and $X$) 
		 have a post value in $\{x,y\}$.  If $\postValueOfInterval{B}\in\{x,y\}$, then the fact that all other boundary intervals
		 $Z$ have post values in $\posts \backslash \{x,y\}$ implies  that
$\transferWithIntervals{A}{\postValueOfInterval{A}}{\postValueOfInterval{\reflectiveMapping(B)}}{\reflectiveMapping(B)}{i}$ is a valid
transfer according 
		 to the rules of the puzzle.  Moreover, as no active intervals with post values in $\{x,y\}$ are covered
		 by static intervals with post values in the same set, the restriction of application of the 
		 mapping to active intervals does not introduce intervals covered by intervals with the same post value
		 within  $(\reflectiveMapping(\alpha_w))_{w=r+1}^{s}$ 
		 
		 After this application of the mapping at $\alpha_{s}$ we have
		 $\postValueOfInterval{X} = \postValueOfInterval{Y}$ and thus we can remove $\lambda_s$ from the resulting transfer
sequence.

		\end{enumerate}

	As with translative noise reduction, these procedures can only remove transfers and thus $|\sigma'|\leq |\sigma|$.
	
	If we express $\sigma(A,B)$ as $\sigma_1 + \omega + \sigma_2$, then the reflective noise reduction yields
	$\sigma' = \sigma_1 + \reflectiveMapping(\omega) +\sigma_2$ which is a valid path that also connects $A$ and $B$.
	
	\end{proof}

==> Proof/ReflectiveCorrectnessProof.tex <==
\begin{proof}\label{proof::reflectiveCorrectness}
	 We consider each case in the above order.
		\begin{enumerate}
		 \item[i.] Firstly, we can apply the mapping $\reflectiveMap{1}{a}{b}$ to $(\alpha_w)_{w=r+1}^{s}$ as no active boundary
intervals in $\omega$ (other than perhaps $B$ and $X$) 
		 have a post value in $\{a,b\}$.  If $\postValueOfInterval{X}\in\{a,b\}$, then the fact that all other boundary intervals
		 $Z$ have post values in $\posts \backslash \{a,b\}$ implies  that
$\transferWithIntervals{\reflectiveMapping(X)}{\postValueOfInterval{\reflectiveMapping(X)}}{\postValueOfInterval{Y}}{Y}{j}$ is a valid
transfer according 
		 to the rules of the puzzle.  Moreover, as no active intervals with post values in $\{a,b\}$ are covered
		 by static intervals with post values in the same set, the restriction of application of the 
		 mapping to active intervals does not introduce intervals covered by intervals with the same post value
		 within  $(\reflectiveMapping(\alpha_w))_{w=r+1}^{s}$ 
		 
		 After this application of the mapping at $\alpha_{r+1}$ we have
		 $\postValueOfInterval{A} = \postValueOfInterval{B}$ and thus we can remove $\lambda_r$ from the resulting transfer
sequence.
		 
		 \item[ii.] Similar to the first case, we can apply the mapping $\reflectiveMap{1}{x}{y}$ to $(\alpha_w)_{w=r+1}^{s}$ as no
active boundary intervals in $\omega$ (other than perhaps $B$ and $X$) 
		 have a post value in $\{x,y\}$.  If $\postValueOfInterval{B}\in\{x,y\}$, then the fact that all other boundary intervals
		 $Z$ have post values in $\posts \backslash \{x,y\}$ implies  that
$\transferWithIntervals{A}{\postValueOfInterval{A}}{\postValueOfInterval{\reflectiveMapping(B)}}{\reflectiveMapping(B)}{i}$ is a valid
transfer according 
		 to the rules of the puzzle.  Moreover, as no active intervals with post values in $\{x,y\}$ are covered
		 by static intervals with post values in the same set, the restriction of application of the 
		 mapping to active intervals does not introduce intervals covered by intervals with the same post value
		 within  $(\reflectiveMapping(\alpha_w))_{w=r+1}^{s}$ 
		 
		 After this application of the mapping at $\alpha_{s}$ we have
		 $\postValueOfInterval{X} = \postValueOfInterval{Y}$ and thus we can remove $\lambda_s$ from the resulting transfer
sequence.

		\end{enumerate}

	As with translative noise reduction, these procedures can only remove transfers and thus $|\sigma'|\leq |\sigma|$.
	
	If we express $\sigma(A,B)$ as $\sigma_1 + \omega + \sigma_2$, then the reflective noise reduction yields
	$\sigma' = \sigma_1 + \reflectiveMapping(\omega) +\sigma_2$ which is a valid path that also connects $A$ and $B$.
	
	\end{proof}

==> Proof/SimplicialHeightVectorBound.tex <==
% !TEX root = ../main.tex
\begin{proof}
	We'll prove this by induction on $q$. When $q=1$, the result  follows from the fact that $\simplexSequenceTerm{1}{c} = 1$ for $c\geq 0$.
	Thus, assume it is true for $q-1$:   the $c$-th term $s_c = \sum_{0 \leq r \leq q} \simplexSequenceTerm{r}{c} \leq \simplexSequenceTerm{q-1}{c+1} + \simplexSequenceTerm{q}{c} = \simplexSequenceTerm{q}{c+1}$.
\end{proof}

==> Proof/Theorem3Precursor.tex <==
% !TEX root = ../main.tex
\begin{proof}\label{proof::theorem3Precursor}
 	Assume the notation and hypotheses within the statement of the lemma.  We will prove this result by induction on $p$ where $p\geq 2$.  In the two-post puzzle, at most one disk can transfer; thus, we impose the condition $j_0 \leq 1$, and any sequence of configurations from distinct source and destination posts must include at least one transfer.   
	
	Assume the claim holds for $p\geq 2$. Let $$\List{1}{m}{C}$$ denote the $e_{p-2}$-grading of $\Path$, and let $\Sum{h}{1}{m}{\Path_h}$ be its $e_{p-2}$-decomposition. Let  $\PathTwo$ denote the cluster path of index $n$
 	\[
 	\Sum{h}{1}{m}{\translativeMap{\Path_h}{C_h}{{\bf 0}^{e_{p-2}}}}. \label{equation::theorem3PathImage}
 	\] This path possesses the following properties:
 	\begin{enumerate}
 		\item\label{condition::fourPostConstraint} the path connects the clusters ${\bf 0}^{e_{p-2}}{\bf a}_{p-2}^{j_{p-2}}$, ${\bf 0}^{e_{p-2}}{\bf c}_{p-2}^{j_{p-2}}$, and ${\bf 0}^{e_{p-2}}{\bf b}_{p-2}^{j_{p-2}}$;
		\item\label{condition::threePostConstraint} for
$h<m$, if $$\translativeMap{\Path_h}{C_h}{{\bf 0}^j} = \List{l(h-1)+1}{l(h)}{\alpha},$$ then
$\alpha_{l(h)} = \alpha_{l(h)+1}$.
	\end{enumerate}
	The disks $\disk{e_{p-2}+1},\ldots,\disk{n}$ generate at least $2M(j_{p-2},p)$ disk transfers according to property
(\ref{condition::fourPostConstraint}), and  $\numberOfTransfers{\sequenceDecomposition{e_{p-2}}{\Path} } \geq M(j_0,2) + 2\sum_{3\leq u \leq p-1}M(j_{u-2},u)$ by the inductive assumption.   Thus, the lower bound
\[
 \numberOfTransfers{\Path} \geq  M(j_0,2) + 2\sum_{3\leq u \leq p}M(j_{u-2},u)
\] holds.
\end{proof}


==> Proof/TranslativeCorrectness.tex <==
%!TEX root = ../main.tex
\begin{proof}\label{proof::translativeCorrectness} We consider the cases in the above order.
	
		\begin{enumerate}
			\item[i. $(q=r)$] No transfers involving post $q$ occur in 
	    \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1}. 
	    Moreover, as both $\lambda_b$ is a transfer  with source post $q$ 
	    (and $\lambda_c$ is a transfer with target post $q$) no boundary intervals of index 
	    $k\ (k>j)$ can exist 
	    in \subpathBySequenceIndices{b}{c}{\sigma}.
	    
		Thus, we can replace the subsequence of intervals $\listKernel{x}{I}{y}$  with the single-element list $(A)$
		( and remove the appropriate transfers) and not violate any rules of the puzzle in the resulting path.  
		
		\item[ii. $(q\neq r)$]We assumed that no transfers include the post $q$ 
			in  \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1}.  
			Moreover, we assumed that no boundary intervals have post value $q$ 
			in  \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1}.  These two assumptions allow the disk 
			\disk{j} to occupy post $q$ within \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1} and transfer to post $r$ 
			at transfer $\lambda_c$.
			
			\item[iii. $(q\neq r)$]We assumed that no transfers include the post $r$ 
			in  \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1}.  
			Moreover, we assumed that no boundary intervals have post value $r$ 
			in  \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1}.  These two assumptions allow the disk 
			\disk{j} to occupy post $r$ within \subpathByDisk{\subpathBySequenceIndices{b}{c}{\sigma}}{j-1} and transfer to post $r$ 
			at transfer $\lambda_b$.
	
		\end{enumerate}

				
			
	\end{proof}

==> Theorem/1.tex <==
% !TEX root = ../main.tex
\begin{theorem}\label{theorem::1}
	Let $i,j\in \nSet{n}$ where $i\leq j$, and let $C \in \clusterSet{i}$.  If the clusters $A,B \in \clusterSetOfCluster{j}{C}$, then every minimal
cluster walk $\clusterSequence{\mu}{A}{B} \subseteq \clusterSetOfCluster{j}{C}$.
\end{theorem}


==> Theorem/2.tex <==
% !TEX root = ../pToH.tex
\begin{theorem}\label{theorem::2}
 Let $j\in \nSet{n}$, and let $a,b\in\posts$ where $a\neq b$. Let the clusters $A,B\in \clusterSet{j}$ where the cluster $A =
\canonicalCluster{a}{1}{j-1}{\bf a}$, and the cluster $B =
\canonicalCluster{a}{1}{j-1}{\bf b}$.   

For a fixed $m\in \nSet{\posts-2}$, assume $\{c_1,\ldots,c_m\} \subset {\posts-\{a,b\}\choose m}$, and assume the cluster $C_w = \canonicalCluster{a}{1}{j-1}{\bf c}_w$ for each $w\in \nSet{m}$.


Define $c_{m+1} = b$, and let $\alpha\in\clusterSetOfCluster{n}{A}$ be such that  the identity
\[
\reflect[j]{\alpha}{c_{w}}{c_{w+1}} = \alpha
\] for $w\in \nSet{m}$.
For a fixed $\beta\in\clusterSetOfCluster{n}{B}$, let $\clusterSequence{\nu}{\alpha}{\beta}$ denote a  cluster walk connecting $\alpha$ and $\beta$ with $j$-grading 
$$\sequenceDecomposition{j}{\nu} =\left(A, \listKernel{C}{1}{m}, B\right).$$  
Then, there exists a cluster walk 
$\clusterSequence{\mu}{\alpha}{\beta}$ possesses the $j$-grading 
\[
 \sequenceDecomposition{j}{\mu} = (A,B),
\] and $\numberOfStates{\mu} = \numberOfStates{\nu}-m$
\end{theorem}


==> Theorem/3.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
\begin{theorem}\label{theorem::intermediateTowerCondition}

	Let $\clusterSequence{\Path}{{\bf 0}^n}{{\bf 1}^n}$ be an acyclic cluster path.
		Define $K_2 = \{1\}$, and let $\sum_{3\leq q \leq p}K_q$ be a partition of $\{2,\ldots,n\}$. 
 Moreover, for each $q\in\{3,\ldots,p\}$, assume that
		\begin{enumerate}
			\item $k_q=\left|\postSetByDiskIndex{K_q}\right|$; and 
			\item there exists a cluster $\alpha_{s(q)}$ in the cluster path in
which every disk with  index in $K_q$ occupies the same post in $\alpha_{s(q)}$, and $\alpha_{s(q)} \notin
\clusterSetOfCluster{n}{{\bf 0}^{u_q}}\cup
\clusterSetOfCluster{n}{{\bf 1}^{u_q}}$.
 		\end{enumerate}
	Then, the inequality 
	\[
	 \numberOfTransfers{\Path} \geq M(1,2) + 2\sum_{3\leq q \leq p}M(k_q,q)
	\] holds.
% 	\end{enumerate}

	
\end{theorem}


==> Theorem/4.tex <==
\begin{theorem}\label{theorem::4}
 
\end{theorem}


==> Theorem/IntermediateTowerBound.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
\begin{theorem}\label{theorem::intermediateTowerBound}

    Assume the notation in Definition \ref{definition::regularity}.
    
	Let $\clusterWalk{\Path}{A}{B}$ be a regular cluster walk of index $n$ with parts $\mathcal{K} = \List{K}{1}{y}$ (of order $y$) and spectrum $(r_q)_{q=1}^{y}$. 
	Then, the inequality 
	\[
	 \numberOfTransfers{\Path} \geq   \sum_{1\leq q \leq y }\parentheses{c(q)-1}\fsBound{k_q}{r_q}
	\] holds.
% 	\end{enumerate}

	
\end{theorem}


==> Theorem/ReflectiveReduction.tex <==
\begin{theorem}\label{theorem::reflectiveReduction}
 
\end{theorem}


==> Theorem/RegularPathsTheorem.tex <==
%!TEX root = ../main.tex
\begin{theorem}[Regular Paths]
	Let $\sigma$ be a path, and let $\left(\subTower{l_0}{r_0},\ldots,\subTower{l_c}{r_c}\right)$ be the sub-tower list of $\sigma$; moreover, assume that $\$
\end{theorem}

==> Theorem/Theorem1.tex <==
\begin

==> Theorem/TranslativeReduction.tex <==
\begin{theorem}\label{theorem::translativeReduction}
 
\end{theorem}


==> Theorem/TriangleInequalityCorollary.tex <==
% !TEX root = ../../HanoiNotes/HanoiNotes.tex
\begin{corollary}
For any $\beta\in\clusterSetOfCluster{n}{B}$, a minimal cluster walk
$\clusterSequence{\mu}{\canonicalCluster{a}{1}{j-1}{\bf a}^{n-j+1}}{\beta}$ possesses the $j$-grading 
\[
 \sequenceDecomposition{j}{\mu} = (A,B).
\]
\end{corollary}

\begin{proof}
This follows from the fact that 
\[
\reflect[j]{\canonicalCluster{a}{1}{j-1}{\bf a}^{n-j+1}}{c}{d} = {\bf a}^{n}
\] when $a\neq c$ and $a\neq d$.
\end{proof}

==> pToHDefinitions.tex <==
%!TEX root = ./sToH.tex

\section{Cluster Spaces}
Our first goal is to present the Puzzle within the mathematical context of a \emph{cluster space}: a hierarchical partitioning  of the state space of disk configurations.  To this end, we will first consider a few definitions describing this state space.   We will first consider the \emph{state graph} of the Puzzle on $n$ disks and $p$ posts; we will define the state graph to be the set pair
	\[
		\stateGraph{n}{p} = (S, E).
	\] The vertex set $S$,
	\[
		S = \{\String{1}{n}{a} \mid a_i \in \posts\},
	\] comprises all possible disk configurations of $n$ disks on $p$ posts.  The edge set $E$ includes a vertex pair $(u,v)$ if and only if the  configurations $u$ and $v$ differ by a valid disk transfer (according to the rules of the Puzzle).  These graphs have been studied by numerous authors over the past decades, and various authors have demonstrated the surprisingly deep connections between these state graphs and  well-known mathematical structures such as Pascal's Triangle and Sierpinski's Gasket.  
	
	 It is known that these graphs are connected for all $n\in \naturals_0$ when $p\geq 3$; thus, in the light of our task to analyze the transfer a tower from one post to another, we can study the {\em walks} in the state graphs that connect vertices whose configurations correspond to towers on different posts.  We will proceed by introducing another object (see \cite{Rukhin}), a \emph{walk tree}, to be a rooted, vertex-labelled tree that represents a walk (possibly with repeated configurations) within the state graph (see Figure \ref{figure::pathTreeExample}). By its construction, a walk tree admits a subtree i.) for each transfer of the largest disk,  and ii.) for each repeated configuration.


\input{./Definition/PathTree}

	\begin{figure}
		\begin{center}
		\input{./Figure/pathTreeDefinition}
		\end{center}
		\caption{A Cluster Walk Tree}{Figure 1 is an illustrated example of a walk tree  of the configuration sequence $(000,001,001,021,022,122,122,022)$ of length $s=8$ with three disks and three posts.  The walk tree is recursively constructed  with $m=5$ subtrees indexed by $\parentheses{u(h)}_{h=1}^{5} = \parentheses{1,3,6,7,8}$.}\label{figure::pathTreeExample}
	\end{figure}
	One can extract the generating sequence of disk configurations by traversing each branch in order from left-to-right.  Hereafter, the examples in this manuscript will forego writing the actual sequence and represent the sequence by its walk tree.
	
	From the tree representations of configuration sequences,  a  hierarchical partitioning of the state space of disk configurations naturally presents itself;  this partitioning of the state space motivates the next definition.

\input{./Definition/Cluster}


{For any cluster $A$ of index $j \ (j\geq 0)$ and for any fixed $k$ with $k\geq j$, an inductive counting argument yields
$|\clusterSetOfCluster{k,p}{A}| = p^{k-j}$. }

Our next definition captures the notion of adjacent disk configurations within the language of clusters.

\input{./Definition/ClusterPair}


{Assume $A,B\in \clusterSet{j}$  form an  $i$-adjacent cluster pair $\clusterPair[i]{A}{B}$ where $\disk{i}$ transfers to and from posts $a$ and $b$ (where $a\neq b$). For any fixed $k$ with $k\geq j$, an inductive counting argument yields
$(p-2)^{k-j}$ $i$--adjacent cluster pairs $\clusterPair[i]{A_k}{B_k}$ where $A_k\in \clusterSetOfCluster{k}{A}$ and $B_k\in \clusterSetOfCluster{k}{B}$:  each disk $\disk{j+1},\ldots,\disk{k}$ must occupy one of the $p-2$ posts in $\posts\backslash\{a,b\}$. }

	The next definition bridges familiar graph-theoretic concepts (e.g., \emph{walk, path}) into the context of clusters.
	
\input{./Definition/ClusterWalk}

\input{./Definition/ClusterWalkConcatenation}

Within the context of walk trees, we can view the $i$-grading of a cluster walk to be the sub-tree  that comprises the first $i$ levels of the walk tree.
\input{./Definition/SequenceDecomposition}

	We now put forth two cluster mappings that will be useful for our analyses in the later sections.
\input{./Definition/ClusterMappings}

Context permitting, we will simply write $\translativeMapNotation(C)$ or $\reflectiveMapNotation(C)$ to express the image of a cluster $C$ under the translative and reflective mappings, respectively.
	
	We will now ensure (under mild assumptions) that the images of cluster walks under these mappings preserve the properties of cluster walks.  
\input{./Lemma/ClusterMappingsOfSequences}
\input{./Proof/ClusterMappingsOfSequences}

	
	 We will  use the established notation found throughout the literature on the Puzzle:  we will write $\minimumMoves{m}{q}$ to denote the minimum number of disk transfers required to transfer a tower of order $m$ using $q$ posts.


==> pToHDenoising.tex <==
%!TEX root = ./pToH.tex

\subsection{Denoising Theorems}
	Being acyclic---the property of not traversing a vertex more than once---is an elementary property of shortest paths within the context of graphs.  	
	It is not difficult to see that all minimal cluster walks must be acyclic: if 
	\[
		\List{C}{1}{m}
	\] is a cluster walk where $C_a = C_b$ for some $1\leq a<b \leq m$, then the sequence of clusters 
	\[
		(\listKernel{C}{1}{a}, \listKernel{C}{b+1}{m})
	\] is a cluster walk of length strictly less than $m$ (this argument, in the language of walks on graphs, can be found in most elementary textbooks on graph theory).  
		 
	 We will begin this section by strengthening the acyclic property for minimal cluster walks within the context of cluster spaces.
		\input{./Theorem/1}
		\input{./Proof/1}
		
		We now will now say that a cluster walk $\Path$ of index $j$ is \emph{acyclic} if and only if its $i$-grading 
$\sequenceDecomposition{i}{\Path}$ does not included repeated elements for each $i\in\nSet{j}$.

	One can view the next result, based on the Reflection Principle,  as a constrained triangle inequality within cluster
spaces.
		
		\input{./Theorem/2}
		\input{./Proof/2}
		\input{./Theorem/TriangleInequalityCorollary}
		With this result, our search for minimal cluster paths connecting towers need only consider  paths in which the
largest disk transfers exactly once.	However, before proceeding, consider the following question:
	
	\begin{quotation}
		\emph{If we decide to construct one or more intermediate towers prior to transferring the largest disk from its source post to its destination post, then why is it optimal to complete the transfer of these intermediate tower(s) before proceeding with the transfer of the largest disk?  Why shouldn't one start the transfers within the $(p-1)$-post component of the Frame-Stewart solution prior to the completion of its $p$-post component?}
	\end{quotation}
	
	In the following subsection, we will show that it is indeed the case that one should complete the transfer of each intermediate tower separately.

==> pToHIntroduction.tex <==
%!TEX root = ./pToH.tex

\section{Introduction}
\subsection{Problem Description}
	The Tower of Hanoi Puzzle consists of $n \ (n\in \naturals_0)$ annular disks (no two disks of equal radius) and $p$ posts $(p\geq
2)$ attached to a fixed base.  The puzzle begins with all of the disks stacked on a single post with no larger disk being
stacked atop a smaller disk.  The goal of the puzzle is to transfer the initial ``tower'' of disks to another post
while adhering to the following rules:
	\begin{enumerate}[i.]
	        \item one disk is transferred from the top of one stack to the top of another (possibly empty) stack at each stage of the puzzle, and
	        \item a larger disk cannot be transferred to a post occupied by a smaller disk.
	\end{enumerate}
	See \cite{HinzBook} for a complete summary and history of the Puzzle.
	One prevailing question that has been studied over the past decades is summarized as follows: assuming feasibility, how does one perform the task in the fewest number of disk transfers?
%	\begin{enumerate}[i.]
%		\item For a given number of disks and a given number of posts, is the task feasible while heeding to these rules? 
%		\item Assuming feasibility, how does one perform the task in the fewest number of disk transfers?
%	\end{enumerate} 
	
	This article considers the same question in a generalization of the classic Puzzle where there are  one or more ``towers" of disks. We will introduce $t$ towers $(t\in \naturals)$ on $p$ posts where  $p \geq t+2$.   Each tower of disks is assigned its own color,  and each tower has $n$ disks of sizes $1,\ldots,n$ where $i<j$ implies that  disk $i$ is larger than  disk $j$. Similar to above, we require that no disk (of any color) is atop any smaller or equal-sized disk (of any color). We will define herein the rules of the parallel puzzle in an analogous manner: 
	\begin{enumerate}[i.]
	        \item one or more one disks (of any color) are transferred---each from the top its own stack---to the top of one or more (possibly empty) stacks at each stage of the puzzle, where no two transfers share the same destination stack, and  
	        \item  a larger disk cannot be transferred to a post occupied by a smaller or equal-sized disk.
	\end{enumerate}
	
	  For other parallel variants of the Tower of Hanoi Puzzle (on a single tower of disks, but where more than one disk can be transferred at each stage) see \cite{WU1992241}  and \cite{LU19953}.   We examine the question of finding walks of minimal length within our parallel context, and we establish two results---with constructive proofs---that prescribe necessary properties that minimal-length walks connecting configurations must possess. These results can be iteratively applied to a given a walk in the state space  connecting arbitrary, valid configurations (e.g., a learning episode of a  reinforcement learning procedure within the context of the Tower of Hanoi Puzzle;  e.g, see \cite{langleyLTS}, \cite{neurIPS},   \cite{BackwardForward}); these results may
	  1.)  potentially reduce the size of the search space for finding walks of minimal  length connecting the configurations, and  
	  2.) decide how this reduced search space should be traversed by a walk of minimal length.

%  When considering the task of finding minimum-length walks in the Tower of Hanoi Puzzle (for both the classical and our parallel version), we need only consider walks that are invariant under the applications of these results.
	
	\subsection{Article Summary}
 The aim of this article is as follows:
\begin{enumerate}[i.]
			\item It formally encapsulates the Parallel Tower of Hanoi Puzzle in a  finite metric space on graphs, words, and sets of words (\emph{clusters}). 
			\item Two theorems---a theorem on acyclicity, and a conditional  triangle inequality---are presented.   These results are generalizations of the results from
\cite{Rukhin}; and the prescribe necessary properties of minimal-length walks within this mathematical framework.			
		\end{enumerate}
			 
	



\subsection{Notation}


	The domain of all variables is the set of  non-negative integers.  Throughout, we use $n$, $p$, and $t$  to denote the number of disks, posts, and towers, respectively.

For any fixed positive integer $m$, we let \nSet{m} denote the set of the first $m$ positive integers.  We 
write \nZeroSet{m} to denote the set $\nSet{m} \cup \{0\}.$ Furthermore, we'll write $\nSetOpen{m}$ and $\nZeroSetOpen{m}$ to denote the sets $\nSet{m-1}$ and $\nZeroSet{m-1}$, respectively. 
We will define the set of $p$ posts to be \posts. 

Assume $\List{X}{i}{i+k}$ is a
subsequence of $k+1$ contiguous elements within the sequence $\List{X}{1}{m}$ (e.g., a subsequence of contiguous symbols in a string, a
subsequence of  adjacent disk configurations). Should the case arise where $k < 0$,  we will assume that the
subsequence \List{X}{i}{i+k} is the empty
sequence (e.g, the empty string $\epsilon$, the empty subsequence).

For a fixed $t$, we will write $\graded{1}^t =\List{1}{}{} \in \naturals^{t}$, and for $j\in \naturals_0$, we will write $j\cdot\graded{1}^t = \List{j}{}{} \in \naturals_0^t$. Context permitting, we will omit the superscript.

Assume that $\graded{i}, \graded{j} \in \naturals_0^t$ where $\graded{i} = \parentheses{i_u}_{u\in \nSet{t}}$ and  $\graded{j} = \parentheses{j_u}_{u\in \nSet{t}}$. We will say that $\graded{i} \preceq \graded{j}$ (equivalently, $\graded{j} \succeq \graded{i}$) if and only if $i_u \leq j_u$ for each $u\in \nSet{t}$. We will also write $\graded{i} \prec \graded{j}$  (equivalently, $\graded{j} \succ \graded{i}$)  if the inequality $i_u < j_u$ (equivalently, $i_u>j_u$) holds for at least one  index $u$. 

We assume that each of the $t$ towers is assigned its own {\sl color}. We will write $\disk{u,j}$ to denote the $j$-th largest disk of color $u$ ($j\in \nSet{n}, u \in \nSet{t}$).  We will represent a configuration of $nt$ disks as $t\times n$ matrix over the set of posts $\posts$:  the matrix 
\[
\begin{bmatrix}
    a_{1,1}  & \dots  & a_{1,n} \\
%    a_{2,1} & \dots  & a_{2,n} \\
    \vdots  & \ddots & \vdots \\
    a_{t,1}  & \dots  &a_{t,n}
\end{bmatrix}
\] encodes a configuration of $t$ towers, each with $n$ disks,  on $p$ posts where the disk $\disk{u,j}$ occupies the post $a_{u,j}$; the largest disks of each color occupy the posts in the in the first (left-most) column, and the post configurations of the smaller disks are listed by column  in decreasing size from left to  right.

==> pToHNotation.tex <==
%!TEX root = ./pToH.tex

	The domain of all variables is the set of  non-negative integers.  Throughout, we use $n$, $p$, and $t$  to denote the number of disks, posts, and towers, respectively.

For any fixed positive integer $m$, we let \nSet{m} denote the set of the first $m$ positive integers.  We 
write \nZeroSet{m} to denote the set $\nSet{m} \cup \{0\}.$ Furthermore, we'll write $\nSetOpen{m}$ and $\nZeroSetOpen{m}$ to denote the sets $\nSet{m-1}$ and $\nZeroSet{m-1}$, respectively. 
We will define the set of $p$ posts to be \posts. 

Assume $\List{X}{i}{i+k}$ is a
subsequence of $k+1$ contiguous elements within the sequence $\List{X}{1}{m}$ (e.g., a subsequence of contiguous symbols in a string, a
subsequence of  adjacent disk configurations). Should the case arise where $k < 0$,  we will assume that the
subsequence \List{X}{i}{i+k} is the empty
sequence (e.g, the empty string $\epsilon$, the empty subsequence).

For a fixed $t$, we will write $\graded{1}^t =\List{1}{}{} \in \naturals^{t}$, and for $j\in \naturals_0$, we will write $j\cdot\graded{1}^t = \List{j}{}{} \in \naturals_0^t$. Context permitting, we will omit the superscript.

Assume that $\graded{i}, \graded{j} \in \naturals_0^t$ where $\graded{i} = \parentheses{i_u}_{u\in \nSet{t}}$ and  $\graded{j} = \parentheses{j_u}_{u\in \nSet{t}}$. We will say that $\graded{i} \preceq \graded{j}$ (equivalently, $\graded{j} \succeq \graded{i}$) if and only if $i_u \leq j_u$ for each $u\in \nSet{t}$. We will also write $\graded{i} \prec \graded{j}$  (equivalently, $\graded{j} \succ \graded{i}$)  if the inequality $i_u < j_u$ (equivalently, $i_u>j_u$) holds for at least one  index $u$. 

We assume that each of the $t$ towers is assigned its own {\sl color}. We will write $\disk{u,j}$ to denote the $j$-th largest disk of color $u$ ($j\in \nSet{n}, u \in \nSet{t}$).  We will represent a configuration of $nt$ disks as $t\times n$ matrix over the set of posts $\posts$:  the matrix 
\[
\begin{bmatrix}
    a_{1,1}  & \dots  & a_{1,n} \\
%    a_{2,1} & \dots  & a_{2,n} \\
    \vdots  & \ddots & \vdots \\
    a_{t,1}  & \dots  &a_{t,n}
\end{bmatrix}
\] encodes a configuration of $t$ towers, each with $n$ disks,  on $p$ posts where the disk $\disk{u,j}$ occupies the post $a_{u,j}$; the largest disks of each color occupy the posts in the in the first (left-most) column, and the post configurations of the smaller disks are listed by column  in decreasing size from left to  right.

%\input{sToHNotationSummary}


==> pToHOutline.tex <==



\section{Introduction}
\subsection{Problem Description}
	The Tower of Hanoi Puzzle consists of $n \ (n\in \naturals_0)$ annular disks (no two disks of equal radius) and $p$ posts $(p\geq
2)$ attached to a fixed base.  The puzzle begins with all of the disks stacked on a single post with no larger disk being
stacked atop a smaller disk.  The goal of the puzzle is to transfer the initial ``tower'' of disks to another post
while adhering to the following rules:
	\begin{enumerate}[i.]
	        \item one disk is transferred from the top of one stack to the top of another (possibly empty) stack at each stage of the puzzle, and
	        \item a larger disk cannot be transferred to a post occupied by a smaller disk.
	\end{enumerate}
	See \cite{HinzBook} for a complete summary and history of the Puzzle.
	One prevailing question that has been studied over the past decades is summarized as follows: assuming feasibility, how does one perform the task in the fewest number of disk transfers?
%	\begin{enumerate}[i.]
%		\item For a given number of disks and a given number of posts, is the task feasible while heeding to these rules? 
%		\item Assuming feasibility, how does one perform the task in the fewest number of disk transfers?
%	\end{enumerate} 
	
	This article considers the same question in a generalization of the classic Puzzle where there are  one or more ``towers" of disks. We will introduce $t$ towers $(t\in \naturals)$ on $p$ posts where  $p \geq t+2$.   Each tower of disks is assigned its own color,  and each tower has $n$ disks of sizes $1,\ldots,n$ where $i<j$ implies that  disk $i$ is larger than  disk $j$. Similar to above, we require that no disk (of any color) is atop any smaller or equal-sized disk (of any color). We will define herein the rules of the parallel puzzle in an analogous manner: 
	\begin{enumerate}[i.]
	        \item one or more one disks (of any color) are transferred---each from the top its own stack---to the top of one or more (possibly empty) stacks at each stage of the puzzle, where no two transfers share the same destination stack, and  
	        \item  a larger disk cannot be transferred to a post occupied by a smaller or equal-sized disk.
	\end{enumerate}
	
	  For other parallel variants of the Tower of Hanoi Puzzle (on a single tower of disks, but where more than one disk can be transferred at each stage) see \cite{WU1992241}  and \cite{LU19953}.   We examine the question of finding walks of minimal length within our parallel context, and we establish two results---with constructive proofs---that prescribe necessary properties that minimal-length walks connecting configurations must possess. These results can be iteratively applied to a given a walk in the state space  connecting arbitrary, valid configurations (e.g., a learning episode of a  reinforcement learning procedure within the context of the Tower of Hanoi Puzzle;  e.g, see \cite{langleyLTS}, \cite{neurIPS},   \cite{BackwardForward}); these results may
	  1.)  potentially reduce the size of the search space for finding walks of minimal  length connecting the configurations, and  
	  2.) decide how this reduced search space should be traversed by a walk of minimal length.

%  When considering the task of finding minimum-length walks in the Tower of Hanoi Puzzle (for both the classical and our parallel version), we need only consider walks that are invariant under the applications of these results.
	
	\subsection{Article Summary}
 The aim of this article is as follows:
\begin{enumerate}[i.]
			\item It formally encapsulates the Parallel Tower of Hanoi Puzzle in a  finite metric space on graphs, words, and sets of words (\emph{clusters}). 
			\item Two theorems---a theorem on acyclicity, and a conditional  triangle inequality---are presented.   These results are generalizations of the results from
\cite{Rukhin}; and the prescribe necessary properties of minimal-length walks within this mathematical framework.			
		\end{enumerate}
			 
	


\subsection{Notation}


	The domain of all variables is the set of  non-negative integers.  Throughout, we use $n$, $p$, and $t$  to denote the number of disks, posts, and towers, respectively.

For any fixed positive integer $m$, we let \nSet{m} denote the set of the first $m$ positive integers.  We 
write \nZeroSet{m} to denote the set $\nSet{m} \cup \{0\}.$ Furthermore, we'll write $\nSetOpen{m}$ and $\nZeroSetOpen{m}$ to denote the sets $\nSet{m-1}$ and $\nZeroSet{m-1}$, respectively. 
We will define the set of $p$ posts to be \posts. 

Assume $\List{X}{i}{i+k}$ is a
subsequence of $k+1$ contiguous elements within the sequence $\List{X}{1}{m}$ (e.g., a subsequence of contiguous symbols in a string, a
subsequence of  adjacent disk configurations). Should the case arise where $k < 0$,  we will assume that the
subsequence \List{X}{i}{i+k} is the empty
sequence (e.g, the empty string $\epsilon$, the empty subsequence).

For a fixed $t$, we will write $\graded{1}^t =\List{1}{}{} \in \naturals^{t}$, and for $j\in \naturals_0$, we will write $j\cdot\graded{1}^t = \List{j}{}{} \in \naturals_0^t$. Context permitting, we will omit the superscript.

Assume that $\graded{i}, \graded{j} \in \naturals_0^t$ where $\graded{i} = \parentheses{i_u}_{u\in \nSet{t}}$ and  $\graded{j} = \parentheses{j_u}_{u\in \nSet{t}}$. We will say that $\graded{i} \preceq \graded{j}$ (equivalently, $\graded{j} \succeq \graded{i}$) if and only if $i_u \leq j_u$ for each $u\in \nSet{t}$. We will also write $\graded{i} \prec \graded{j}$  (equivalently, $\graded{j} \succ \graded{i}$)  if the inequality $i_u < j_u$ (equivalently, $i_u>j_u$) holds for at least one  index $u$. 

We assume that each of the $t$ towers is assigned its own {\sl color}. We will write $\disk{u,j}$ to denote the $j$-th largest disk of color $u$ ($j\in \nSet{n}, u \in \nSet{t}$).  We will represent a configuration of $nt$ disks as $t\times n$ matrix over the set of posts $\posts$:  the matrix 
\[
\begin{bmatrix}
    a_{1,1}  & \dots  & a_{1,n} \\
%    a_{2,1} & \dots  & a_{2,n} \\
    \vdots  & \ddots & \vdots \\
    a_{t,1}  & \dots  &a_{t,n}
\end{bmatrix}
\] encodes a configuration of $t$ towers, each with $n$ disks,  on $p$ posts where the disk $\disk{u,j}$ occupies the post $a_{u,j}$; the largest disks of each color occupy the posts in the in the first (left-most) column, and the post configurations of the smaller disks are listed by column  in decreasing size from left to  right.

%\input{sToHDefinitions}

\section{The Parallel Tower of Hanoi Problem}

In this section, we will establish the mathematical machinery to analyze the state space of disk configurations in a hierarchical manner: we will partition the state space of disk configurations into sets (called {\sl clusters}) that are defined by the arrangement of a prescribed subset of the largest disks.  Afterwards, as was originally done in \cite{Scorer}, we will  represent the parallel state space of configurations in the context of graphs.  We will define the formalism to  analyze walks within these graphs, as well as {\sl cluster walks}: for a pair $(\alpha, \beta)$ of arbitrary configurations within the state space, this machinery will allow us to decide in which subsets of configurations (i.e., the corresponding subsets of vertices in the state graph) that minimal walks connecting $\alpha$ and $\beta$ must be contained. 




\input{Definition/pCluster}

%	\begin{definition}  Let $\graded{j} = \List{j}{1}{t}$ where $j_u \in \nSet{n}$ for each $u\in \nSet{t}$. We define a cluster of grading \graded{j} to the set of configurations in which the disks $\disk{u,i_u}$ are in a fixed configuration for $u\in \nSet{\tau}$ and $i_u\leq j_u$.
%	\end{definition}
%
For $j\in \nSet{n}$, there are $p$ choices to place $\disk{1,j}$, $p-1$ choices to place $\disk{2,j}, \ldots, p-t+1$ choices to place $\disk{t,j}$.  Thus, there are $p^{\falling{t}}$ choices to place the $t$ disks of  index $j$.  Consequently, induction yields  $\parentheses{p^{\falling{t}}}^{j}$ clusters of grading $j\cdot \graded{1}$.



\subsection{EREW-Adjacency (Exclusive Read, Exclusive Write Adjacency) }

In the classical puzzle, two configurations were adjacent if and only if they differed by the valid transfer of a single disk.  We now extend this definition into the parallel context as follows.
\input{Definition/EREWAdjacency}


One consequence of this definition is the {\sl exclusive read/write} property for the parallel Puzzle: if $a_{u,j_u} \neq b_{u,j_u}$ and $a_{v,j_v} \neq b_{v,j_v}$ where $u\neq v$, then $a_{u,j_u} \neq a_{v,j_v}$ and  $b_{u,j_u} \neq b_{v,j_v}$. 

Equipped with this definition of adjacency, we will define the {\sl state graph} of the parallel Puzzle as was done in \cite{Scorer} for the single-tower case (see Figure \ref{figure::stateGraphEx}).

\input{Definition/pStateGraph}



	\begin{figure}[h!]
		\centering	
		\input{./Figure/FourPostsTwoDisksGraph}
		\input{./Figure/FourPostsOneDiskPToH}
		\caption{Illustrated Examples of the graphs $H^{1,2}_4$ and $H^{2,1}_4$; only the edges on the hull of $H^{2,1}_4 \equiv K_{12}$ are presented.}\label{figure::stateGraphEx}
	\end{figure}


We now define a {\sl cluster walk}, and we will equip walks in the parallel state space with a measure in the parallel state space that naturally aligns with the counting measure of the classic Puzzle. To this end,
we will introduce an auxiliary graph object for the parallel Puzzle.

\input{Definition/pTransitionGraph}

As per the rules of the parallel Puzzle, the in-degree and out-degree of any vertex in the transition graph is at most one.

We will now define adjaceny for clusters as follows. 

\input{Definition/pClusterPair}


\input{Definition/pClusterWalk}

We will also define a {\sl valid} sequence of configurations $\List{\alpha}{1}{w}$ analogously (we allow repeated configurations in a valid sequence of configurations).

% a sequence of configurations $\List{A}{1}{w}$ is valid if and only if $A_u = A_{u+1}$ or $\clusterPair[\graded{j}]{A_u}{A_{u+1}}$ for some grading $\graded{j} \in \nSet{n}^t$.



We will define both the {\sl sequence length} and {\sl transfer length} of configuration sequences.    If $\Path = \List{\alpha}{1}{w}$ is a configuration sequence, then its sequence length is defined to be $\numberOfStates{\Path} = w$ (the number of configurations in $\Path$), and its transfer length is defined to be $\transferLength{\Path} = \sum_{1\leq v < w} \tgec{\alpha_v,\alpha_{v+1}}$ (the sum of the number of edges in all transition graphs of $\Path$).   

%We will also write $\numberOfStates{\Path} = w$.


%As in the serial case, we will formulate disk(s) transfers between adjacent configurations in terms of mappings. 


%In order to apply the reflective map to cluster walks in the parallel context, we include an additional definition.


%\begin{definition}
%
%Let $\graded{q},\graded{r} \in \posts^t$ where $\graded{q} = \List{q}{1}{t}$ and $\graded{r} = \List{r}{1}{t}$. 
%% Furthermore,  for $u,v\in \nSet{t}$., assume that $u\neq v$ implies $q_u\neq q_v$ and $r_u\neq r_v$.
%Assume that $u\neq v$ implies $q_u\neq q_v$ ({\sl exclusive read}) and $r_u \neq r_v$ ({\sl exclusive write}); furthermore, if $q_u \neq r_u$, then $q_u\neq r_v$ and $q_v\neq r_u$ for $v\in \nSet{t}$ ({\sl collision avoidance}).
%We will say that (\graded{q},\graded{r}) form an {\sl collision-free, exclusive read/exclusive-write (EREW)}  pair. 
%\end{definition}

In order to establish results on the transfer length of configuration sequences, we will formally prescribe disk transfers as mappings on such sequences. 



\input{Definition/pMappings}


We will now identify a class of mappings that for which the images of valid configuration sequences are themselves valid.

\input{Lemma/pClusterMappings}

\section{Results}

An elementary result of graph theory states that any minimal path in a graph connecting a pair of vertices must be acyclic. 
The first theorem extends the notion of {\sl acyclicity} of minimal walks into the context of parallel cluster walks. 
 


\input{Theorem/p1}
\input{Proof/p1}

The second theorem yields a conditional triangle inequality within the context of parallel clusters.

\input{Theorem/p2}
\input{Proof/p2}


==> pToHParallel.tex <==
%!TEX root = ./pToH.tex

\section{The Parallel Tower of Hanoi Problem}

In this section, we will establish the mathematical machinery to analyze the state space of disk configurations in a hierarchical manner: we will partition the state space of disk configurations into sets (called {\sl clusters}) that are defined by the arrangement of a prescribed subset of the largest disks.  Afterwards, as was originally done in \cite{Scorer}, we will  represent the parallel state space of configurations in the context of graphs.  We will define the formalism to  analyze walks within these graphs, as well as {\sl cluster walks}: for a pair $(\alpha, \beta)$ of arbitrary configurations within the state space, this machinery will allow us to decide in which subsets of configurations (i.e., the corresponding subsets of vertices in the state graph) that minimal walks connecting $\alpha$ and $\beta$ must be contained. 




\input{Definition/pCluster}

%	\begin{definition}  Let $\graded{j} = \List{j}{1}{t}$ where $j_u \in \nSet{n}$ for each $u\in \nSet{t}$. We define a cluster of grading \graded{j} to the set of configurations in which the disks $\disk{u,i_u}$ are in a fixed configuration for $u\in \nSet{\tau}$ and $i_u\leq j_u$.
%	\end{definition}
%
For $j\in \nSet{n}$, there are $p$ choices to place $\disk{1,j}$, $p-1$ choices to place $\disk{2,j}, \ldots, p-t+1$ choices to place $\disk{t,j}$.  Thus, there are $p^{\falling{t}}$ choices to place the $t$ disks of  index $j$.  Consequently, induction yields  $\parentheses{p^{\falling{t}}}^{j}$ clusters of grading $j\cdot \graded{1}$.



\subsection{EREW-Adjacency (Exclusive Read, Exclusive Write Adjacency) }

In the classical puzzle, two configurations were adjacent if and only if they differed by the valid transfer of a single disk.  We now extend this definition into the parallel context as follows.
\input{Definition/EREWAdjacency}


One consequence of this definition is the {\sl exclusive read/write} property for the parallel Puzzle: if $a_{u,j_u} \neq b_{u,j_u}$ and $a_{v,j_v} \neq b_{v,j_v}$ where $u\neq v$, then $a_{u,j_u} \neq a_{v,j_v}$ and  $b_{u,j_u} \neq b_{v,j_v}$. 

Equipped with this definition of adjacency, we will define the {\sl state graph} of the parallel Puzzle as was done in \cite{Scorer} for the single-tower case (see Figure \ref{figure::stateGraphEx}).

\input{Definition/pStateGraph}



	\begin{figure}[h!]
		\centering	
		\input{./Figure/FourPostsTwoDisksGraph}
		\input{./Figure/FourPostsOneDiskPToH}
		\caption{Illustrated Examples of the graphs $H^{1,2}_4$ and $H^{2,1}_4$; only the edges on the hull of $H^{2,1}_4 \equiv K_{12}$ are presented.}\label{figure::stateGraphEx}
	\end{figure}


We now define a {\sl cluster walk}, and we will equip walks in the parallel state space with a measure in the parallel state space that naturally aligns with the counting measure of the classic Puzzle. To this end,
we will introduce an auxiliary graph object for the parallel Puzzle.

\input{Definition/pTransitionGraph}

As per the rules of the parallel Puzzle, the in-degree and out-degree of any vertex in the transition graph is at most one.

We will now define adjaceny for clusters as follows. 

\input{Definition/pClusterPair}


\input{Definition/pClusterWalk}

We will also define a {\sl valid} sequence of configurations $\List{\alpha}{1}{w}$ analogously (we allow repeated configurations in a valid sequence of configurations).

% a sequence of configurations $\List{A}{1}{w}$ is valid if and only if $A_u = A_{u+1}$ or $\clusterPair[\graded{j}]{A_u}{A_{u+1}}$ for some grading $\graded{j} \in \nSet{n}^t$.



We will define both the {\sl sequence length} and {\sl transfer length} of configuration sequences.    If $\Path = \List{\alpha}{1}{w}$ is a configuration sequence, then its sequence length is defined to be $\numberOfStates{\Path} = w$ (the number of configurations in $\Path$), and its transfer length is defined to be $\transferLength{\Path} = \sum_{1\leq v < w} \tgec{\alpha_v,\alpha_{v+1}}$ (the sum of the number of edges in all transition graphs of $\Path$).   

%We will also write $\numberOfStates{\Path} = w$.


%As in the serial case, we will formulate disk(s) transfers between adjacent configurations in terms of mappings. 


%In order to apply the reflective map to cluster walks in the parallel context, we include an additional definition.


%\begin{definition}
%
%Let $\graded{q},\graded{r} \in \posts^t$ where $\graded{q} = \List{q}{1}{t}$ and $\graded{r} = \List{r}{1}{t}$. 
%% Furthermore,  for $u,v\in \nSet{t}$., assume that $u\neq v$ implies $q_u\neq q_v$ and $r_u\neq r_v$.
%Assume that $u\neq v$ implies $q_u\neq q_v$ ({\sl exclusive read}) and $r_u \neq r_v$ ({\sl exclusive write}); furthermore, if $q_u \neq r_u$, then $q_u\neq r_v$ and $q_v\neq r_u$ for $v\in \nSet{t}$ ({\sl collision avoidance}).
%We will say that (\graded{q},\graded{r}) form an {\sl collision-free, exclusive read/exclusive-write (EREW)}  pair. 
%\end{definition}

In order to establish results on the transfer length of configuration sequences, we will formally prescribe disk transfers as mappings on such sequences. 



\input{Definition/pMappings}


We will now identify a class of mappings that for which the images of valid configuration sequences are themselves valid.

\input{Lemma/pClusterMappings}

\section{Results}

An elementary result of graph theory states that any minimal path in a graph connecting a pair of vertices must be acyclic. 
The first theorem extends the notion of {\sl acyclicity} of minimal walks into the context of parallel cluster walks. 
 


\input{Theorem/p1}
\input{Proof/p1}

The second theorem yields a conditional triangle inequality within the context of parallel clusters.

\input{Theorem/p2}
\input{Proof/p2}

%Let $\Path$ denote an arbitrary cluster walk connecting a fixed pair of disk configurations.  The constructive methods within the proofs of these two results can be iteratively applied to $\Path$ to yield a walk $\Path'$ with the property that $\transferLength{\Path'} \leq \transferLength{\Path}$.  It follows that the set of walks that are invariant under the applications of these methods must contain a minimal walk between a fixed pair of configurations; thus, the current research focus of the author is bounding the elements of such sets.

%\section{The \code{Denoise} Method}
%
%\input{Algorithm/pDenoising}

==> pToHResults.tex <==
%!TEX root = ./sToH.tex

\section{Main Results}

		\input{./sToHDenoising}
		%\input{./sToHLowerBoundsRegular}
		%\input{./sToHLowerBoundsIrregular}

